A Meeting Transcription System for an Ad-Hoc Acoustic Sensor Network

We propose a system that transcribes the conversation of a typical meeting scenario that is captured by a set of initially unsynchronized microphone arrays at unknown positions. It consists of subsystems for signal synchronization, including both sampling rate and sampling time offset estimation, diarization based on speaker and microphone array position estimation, multi-channel speech enhancement, and automatic speech recognition. With the estimated diarization information, a spatial mixture model is initialized that is used to estimate beamformer coefficients for source separation. Simulations show that the speech recognition accuracy can be improved by synchronizing and combining multiple distributed microphone arrays compared to a single compact microphone array. Furthermore, the proposed informed initialization of the spatial mixture model delivers a clear performance advantage over random initialization.

==> figures/sro_error.tex <==
% This file was created by tikzplotlib v0.8.4.
\pgfplotsset{compat=1.3}

\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\newcommand{\mydiv}{\raisebox{-0.5ex}{\resizebox{!}{2.ex}{/}}}

\begin{groupplot}[group style={group size=2 by 1, horizontal sep=1.45cm}]
\nextgroupplot[
height=5cm,
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=1/2*\linewidth,
x grid style={white!69.01960784313725!black},
xlabel={\( \displaystyle \text{RMSE} \left(\tau_\varepsilon[\ell]\right) \mydiv \text{samples}\)},
xmajorgrids,
xmin=0, xmax=2,
xtick style={color=black},
xtick={0,0.5,1,1.5,2},
xticklabels={0.0,0.5,1.0,1.5,2.0},
y grid style={white!69.01960784313725!black},
ylabel={\(\displaystyle \text{CDF}\left(\text{RMSE} \left(\tau_\varepsilon[\ell]\right)\right)\)},
ylabel shift = -.1cm,
ymajorgrids,
ymin=-5, ymax=105,
ytick style={color=black},
ytick={0,10,20,30,40,50,60,70,80,90,100}
]
\addplot [line width=1.5pt, color0]
table {%
0 0
0.397210478782654 0
0.406121045351028 0.5
0.415031641721725 0.5
0.4239422082901 1
0.432852774858475 1
0.441763341426849 2
0.450673937797546 2.5
0.459584504365921 3
0.468495070934296 4.5
0.477405667304993 6.5
0.486316233873367 8.5
0.495226800441742 10.5
0.504137396812439 11
0.513047933578491 13.5
0.521958529949188 15.5
0.530869126319885 18.5
0.539779663085938 21
0.548690259456635 23.5
0.557600855827332 25
0.566511392593384 27
0.575421988964081 30.5
0.584332525730133 33.5
0.59324312210083 36
0.602153718471527 37.5
0.611064255237579 39
0.619974851608276 41.5
0.628885447978973 44.5
0.637795984745026 48
0.646706581115723 50.5
0.65561717748642 52
0.664527714252472 54
0.673438310623169 54.5
0.682348847389221 55.5
0.691259443759918 57.5
0.700170040130615 59.5
0.709080576896667 60
0.717991173267365 62
0.726901769638062 64.5
0.735812306404114 66
0.744722902774811 70
0.753633499145508 71.5
0.76254403591156 73.5
0.771454632282257 75
0.780365228652954 78
0.789275765419006 79
0.798186361789703 80
0.807096898555756 81.5
0.816007494926453 82.5
0.82491809129715 83.5
0.833828628063202 85.5
0.842739224433899 86.5
0.851649820804596 87.5
0.860560357570648 88
0.869470953941345 88.5
0.878381550312042 90.5
0.887292087078094 91.5
0.896202683448792 91.5
0.905113220214844 93
0.914023816585541 94
0.922934412956238 94
0.93184494972229 94
0.940755546092987 94
0.949666142463684 95
0.958576679229736 95.5
0.967487275600433 96.5
0.97639787197113 96.5
0.985308408737183 97.5
0.99421900510788 97.5
1.00312960147858 97.5
1.01204013824463 97.5
1.02095067501068 98.5
1.02986133098602 99
1.03877186775208 99.5
1.04768240451813 99.5
1.05659306049347 99.5
1.06550359725952 99.5
1.07441413402557 99.5
1.08332479000092 99.5
1.09223532676697 99.5
1.10114586353302 99.5
1.11005651950836 99.5
1.11896705627441 99.5
1.12787759304047 99.5
1.13678824901581 99.5
1.14569878578186 99.5
1.15460932254791 99.5
1.16351997852325 99.5
1.17243051528931 99.5
1.18134105205536 99.5
1.19025158882141 99.5
1.19916224479675 99.5
1.20807278156281 99.5
1.21698331832886 99.5
1.2258939743042 99.5
1.23480451107025 99.5
1.2437150478363 99.5
1.25262570381165 99.5
1.2615362405777 99.5
1.27044677734375 99.5
1.27935743331909 99.5
1.28826797008514 100
3 100
};

\nextgroupplot[
height=5cm,
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=1/2*\linewidth,
x grid style={white!69.01960784313725!black},
xlabel={max\(\displaystyle \left(\left|\tau_\varepsilon[\ell] - \widehat{\tau}_\varepsilon[\ell]\right|\right)\mydiv\)samples},
xmajorgrids,
xmin=0, xmax=3,
xtick style={color=black},
xtick={0,1,2,3},
xticklabels={0.0,1.0,2.0,3.0},
y grid style={white!69.01960784313725!black},
ylabel={CDF(max\(\displaystyle \left(\left|\tau_\varepsilon[\ell] - \widehat{\tau}_\varepsilon[\ell]\right|\right)\))},
ylabel shift = -.1cm,
ymajorgrids,
ymin=-5, ymax=105,
ytick style={color=black},
ytick={0,10,20,30,40,50,60,70,80,90,100}
]
\addplot [line width=1.5pt, color0]
table {%
0 0
0.157801494002342 0
0.180614903569221 1
0.203428313136101 1.5
0.22624172270298 2.5
0.249055117368698 5
0.271868526935577 9.5
0.294681936502457 12.5
0.317495346069336 14.5
0.340308755636215 16
0.363122165203094 19
0.385935574769974 20
0.408748984336853 22.5
0.431562393903732 25
0.454375803470612 27
0.477189183235168 31
0.50000262260437 34.5
0.522816002368927 42
0.545629441738129 44
0.568442821502686 47.5
0.591256260871887 52.5
0.614069640636444 55
0.636883020401001 58
0.659696459770203 59.5
0.68250983953476 60.5
0.705323278903961 64
0.728136658668518 65.5
0.75095009803772 67
0.773763477802277 67.5
0.796576917171478 69.5
0.819390296936035 71
0.842203736305237 74.5
0.865017116069794 77.5
0.887830555438995 79
0.910643935203552 79.5
0.933457314968109 81.5
0.956270754337311 83.5
0.979084134101868 84.5
1.00189757347107 85.5
1.02471101284027 87.5
1.04752433300018 87.5
1.07033777236938 89
1.09315121173859 91.5
1.11596465110779 92
1.1387779712677 92.5
1.1615914106369 94
1.1844048500061 95
1.20721828937531 95
1.23003160953522 95.5
1.25284504890442 95.5
1.27565848827362 95.5
1.29847180843353 95.5
1.32128524780273 95.5
1.34409868717194 96
1.36691212654114 96.5
1.38972544670105 96.5
1.41253888607025 96.5
1.43535232543945 96.5
1.45816576480865 96.5
1.48097908496857 97
1.50379252433777 97.5
1.52660596370697 97.5
1.54941928386688 97.5
1.57223272323608 98
1.59504616260529 99
1.61785960197449 99
1.6406729221344 99
1.6634863615036 99
1.6862998008728 99
1.709113240242 99
1.73192656040192 99
1.75473999977112 99
1.77755343914032 99
1.80036687850952 99
1.82318019866943 99
1.84599363803864 99
1.86880707740784 99
1.89162039756775 99
1.91443383693695 99
1.93724727630615 99
1.96006071567535 99.5
1.98287403583527 99.5
2.00568747520447 99.5
2.02850079536438 99.5
2.05131435394287 99.5
2.07412767410278 99.5
2.09694123268127 99.5
2.11975455284119 99.5
2.1425678730011 99.5
2.16538143157959 99.5
2.1881947517395 99.5
2.21100807189941 99.5
2.23382163047791 99.5
2.25663495063782 99.5
2.27944827079773 99.5
2.30226182937622 99.5
2.32507514953613 99.5
2.34788870811462 99.5
2.37070202827454 99.5
2.39351534843445 99.5
2.41632890701294 99.5
2.43914222717285 100
3 100
};
\end{groupplot}

\end{tikzpicture}

==> figures/sto_error.tex <==
% This file was created by tikzplotlib v0.8.4.
\pgfplotsset{compat=1.3}

\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\newcommand{\mydiv}{\raisebox{-0.5ex}{\resizebox{!}{2.ex}{/}}}

\begin{axis}[
height=5cm,
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=\linewidth,
x grid style={white!69.01960784313725!black},
xlabel={\(\scriptstyle \left|T_l - \widehat{T}_l\right| \mydiv \)\si{samples}  },
xmajorgrids,
xmin=0, xmax=4,
xtick style={color=black},
xtick={0.0,0.5,1.0,1.5,2.0,2.5,3.0,3.5,4.0,4.5,5.0},
xticklabels={0.0,0.5,1.0,1.5,2.0,2.5,3.0,3.5,4.0,4.5,5.0},
y grid style={white!69.01960784313725!black},
ylabel={CDF\(\scriptstyle \left(\left|T_l - \widehat{T}_l\right|\right)  \mydiv \%\)},
ylabel shift = -.1cm,
ymajorgrids,
ymin=-5, ymax=105,
ytick style={color=black},
ytick={0,10,20,30,40,50,60,70,80,90,100}
]
\addplot [line width=1.5pt, color0]
table {%
0.0116759383136014 0
0.0501835487151675 1.5
0.0886911591167336 4.5
0.1271987695183 7
0.165706379919866 10
0.204213990321432 12.5
0.242721600722998 15.5
0.281229211124564 16.5
0.31973682152613 18.5
0.358244431927697 20
0.396752042329263 25
0.435259652730829 25.5
0.473767263132395 26
0.512274873533961 27
0.550782483935527 29.5
0.589290094337093 33
0.627797704738659 35
0.666305315140226 36
0.704812925541792 38
0.743320535943358 39
0.781828146344924 41.5
0.82033575674649 45
0.858843367148056 45.5
0.897350977549622 48.5
0.935858587951188 51
0.974366198352755 53.5
1.01287380875432 55
1.05138141915589 56.5
1.08988902955745 58.5
1.12839663995902 59
1.16690425036059 59.5
1.20541186076215 63
1.24391947116372 66
1.28242708156528 67.5
1.32093469196685 69
1.35944230236842 71.5
1.39794991276998 73.5
1.43645752317155 76
1.47496513357311 76.5
1.51347274397468 77
1.55198035437625 78.5
1.59048796477781 79
1.62899557517938 79.5
1.66750318558094 80.5
1.70601079598251 81
1.74451840638408 82
1.78302601678564 83
1.82153362718721 83.5
1.86004123758878 84.5
1.89854884799034 85
1.93705645839191 85
1.97556406879347 85.5
2.01407167919504 86
2.05257928959661 86
2.09108689999817 87
2.12959451039974 88
2.1681021208013 88.5
2.20660973120287 89.5
2.24511734160444 89.5
2.283624952006 90
2.32213256240757 90.5
2.36064017280914 91
2.3991477832107 91
2.43765539361227 91.5
2.47616300401383 91.5
2.5146706144154 91.5
2.55317822481697 92
2.59168583521853 92.5
2.6301934456201 92.5
2.66870105602166 93
2.70720866642323 93
2.7457162768248 93.5
2.78422388722636 93.5
2.82273149762793 93.5
2.86123910802949 93.5
2.89974671843106 94
2.93825432883263 94
2.97676193923419 94.5
3.01526954963576 94.5
3.05377716003733 94.5
3.09228477043889 94.5
3.13079238084046 94.5
3.16929999124202 94.5
3.20780760164359 94.5
3.24631521204516 94.5
3.28482282244672 94.5
3.32333043284829 94.5
3.36183804324985 95.5
3.40034565365142 96
3.43885326405299 96
3.47736087445455 97
3.51586848485612 98
3.55437609525768 98
3.59288370565925 98.5
3.63139131606082 98.5
3.66989892646238 99.5
3.70840653686395 99.5
3.74691414726552 99.5
3.78542175766708 99.5
3.82392936806865 99.5
3.86243697847021 100
5 100
};
\end{axis}

\end{tikzpicture}

==> figures/sync_error.tex <==
% This file was created by tikzplotlib v0.8.4.
\pgfplotsset{compat=1.3}

\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\newcommand{\mydiv}{\raisebox{-0.5ex}{\resizebox{!}{2.ex}{/}}}

\begin{groupplot}[group style={group size=2 by 1, horizontal sep=1.45cm}]
\nextgroupplot[
height=4cm,
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=1/2*\linewidth,
x grid style={white!69.01960784313725!black},
xlabel={\( \displaystyle \text{RMSE} \left(\tau_\varepsilon[\ell]\right) \mydiv \text{samples}\)},
xmajorgrids,
xmin=0, xmax=2.005,
xtick style={color=black},
xtick={0,0.5,1,1.5,2},
xticklabels={0.0,0.5,1.0,1.5,2.0},
y grid style={white!69.01960784313725!black},
ylabel={\(\displaystyle \text{CDF}\left(\text{RMSE} \left(\tau_\varepsilon[\ell]\right)\right)\)},
ylabel shift = -.1cm,
ymajorgrids,
ymin=-5, ymax=105,
ytick style={color=black},
ytick={0,20,40,60,80,100}
]
\addplot [line width=1.5pt, color0]
table {%
0 0
0.397210478782654 0
0.406121045351028 0.5
0.415031641721725 0.5
0.4239422082901 1
0.432852774858475 1
0.441763341426849 2
0.450673937797546 2.5
0.459584504365921 3
0.468495070934296 4.5
0.477405667304993 6.5
0.486316233873367 8.5
0.495226800441742 10.5
0.504137396812439 11
0.513047933578491 13.5
0.521958529949188 15.5
0.530869126319885 18.5
0.539779663085938 21
0.548690259456635 23.5
0.557600855827332 25
0.566511392593384 27
0.575421988964081 30.5
0.584332525730133 33.5
0.59324312210083 36
0.602153718471527 37.5
0.611064255237579 39
0.619974851608276 41.5
0.628885447978973 44.5
0.637795984745026 48
0.646706581115723 50.5
0.65561717748642 52
0.664527714252472 54
0.673438310623169 54.5
0.682348847389221 55.5
0.691259443759918 57.5
0.700170040130615 59.5
0.709080576896667 60
0.717991173267365 62
0.726901769638062 64.5
0.735812306404114 66
0.744722902774811 70
0.753633499145508 71.5
0.76254403591156 73.5
0.771454632282257 75
0.780365228652954 78
0.789275765419006 79
0.798186361789703 80
0.807096898555756 81.5
0.816007494926453 82.5
0.82491809129715 83.5
0.833828628063202 85.5
0.842739224433899 86.5
0.851649820804596 87.5
0.860560357570648 88
0.869470953941345 88.5
0.878381550312042 90.5
0.887292087078094 91.5
0.896202683448792 91.5
0.905113220214844 93
0.914023816585541 94
0.922934412956238 94
0.93184494972229 94
0.940755546092987 94
0.949666142463684 95
0.958576679229736 95.5
0.967487275600433 96.5
0.97639787197113 96.5
0.985308408737183 97.5
0.99421900510788 97.5
1.00312960147858 97.5
1.01204013824463 97.5
1.02095067501068 98.5
1.02986133098602 99
1.03877186775208 99.5
1.04768240451813 99.5
1.05659306049347 99.5
1.06550359725952 99.5
1.07441413402557 99.5
1.08332479000092 99.5
1.09223532676697 99.5
1.10114586353302 99.5
1.11005651950836 99.5
1.11896705627441 99.5
1.12787759304047 99.5
1.13678824901581 99.5
1.14569878578186 99.5
1.15460932254791 99.5
1.16351997852325 99.5
1.17243051528931 99.5
1.18134105205536 99.5
1.19025158882141 99.5
1.19916224479675 99.5
1.20807278156281 99.5
1.21698331832886 99.5
1.2258939743042 99.5
1.23480451107025 99.5
1.2437150478363 99.5
1.25262570381165 99.5
1.2615362405777 99.5
1.27044677734375 99.5
1.27935743331909 99.5
1.28826797008514 100
3 100
};

\nextgroupplot[
height=4cm,
minor xtick={},
minor ytick={},
tick align=outside,
tick pos=left,
width=1/2*\linewidth,
x grid style={white!69.01960784313725!black},
xlabel={\(\scriptstyle \left|T_l - \widehat{T}_l\right| \mydiv \)\si{samples}  },
xmajorgrids,
xmin=0, xmax=4.005,
xtick style={color=black},
xtick={0.0,1.0,2.0,3.0,4.0,5.0},
xticklabels={0.0,1.0,2.0,3.0,4.0,5.0},
y grid style={white!69.01960784313725!black},
ylabel={CDF\(\scriptstyle \left(\left|T_l - \widehat{T}_l\right|\right)  \mydiv \%\)},
ylabel shift = -.1cm,
ymajorgrids,
ymin=-5, ymax=105,
ytick style={color=black},
ytick={0,20,40,60,80,100}
]
\addplot [line width=1.5pt, color0]
table {%
	0.0116759383136014 0
	0.0501835487151675 1.5
	0.0886911591167336 4.5
	0.1271987695183 7
	0.165706379919866 10
	0.204213990321432 12.5
	0.242721600722998 15.5
	0.281229211124564 16.5
	0.31973682152613 18.5
	0.358244431927697 20
	0.396752042329263 25
	0.435259652730829 25.5
	0.473767263132395 26
	0.512274873533961 27
	0.550782483935527 29.5
	0.589290094337093 33
	0.627797704738659 35
	0.666305315140226 36
	0.704812925541792 38
	0.743320535943358 39
	0.781828146344924 41.5
	0.82033575674649 45
	0.858843367148056 45.5
	0.897350977549622 48.5
	0.935858587951188 51
	0.974366198352755 53.5
	1.01287380875432 55
	1.05138141915589 56.5
	1.08988902955745 58.5
	1.12839663995902 59
	1.16690425036059 59.5
	1.20541186076215 63
	1.24391947116372 66
	1.28242708156528 67.5
	1.32093469196685 69
	1.35944230236842 71.5
	1.39794991276998 73.5
	1.43645752317155 76
	1.47496513357311 76.5
	1.51347274397468 77
	1.55198035437625 78.5
	1.59048796477781 79
	1.62899557517938 79.5
	1.66750318558094 80.5
	1.70601079598251 81
	1.74451840638408 82
	1.78302601678564 83
	1.82153362718721 83.5
	1.86004123758878 84.5
	1.89854884799034 85
	1.93705645839191 85
	1.97556406879347 85.5
	2.01407167919504 86
	2.05257928959661 86
	2.09108689999817 87
	2.12959451039974 88
	2.1681021208013 88.5
	2.20660973120287 89.5
	2.24511734160444 89.5
	2.283624952006 90
	2.32213256240757 90.5
	2.36064017280914 91
	2.3991477832107 91
	2.43765539361227 91.5
	2.47616300401383 91.5
	2.5146706144154 91.5
	2.55317822481697 92
	2.59168583521853 92.5
	2.6301934456201 92.5
	2.66870105602166 93
	2.70720866642323 93
	2.7457162768248 93.5
	2.78422388722636 93.5
	2.82273149762793 93.5
	2.86123910802949 93.5
	2.89974671843106 94
	2.93825432883263 94
	2.97676193923419 94.5
	3.01526954963576 94.5
	3.05377716003733 94.5
	3.09228477043889 94.5
	3.13079238084046 94.5
	3.16929999124202 94.5
	3.20780760164359 94.5
	3.24631521204516 94.5
	3.28482282244672 94.5
	3.32333043284829 94.5
	3.36183804324985 95.5
	3.40034565365142 96
	3.43885326405299 96
	3.47736087445455 97
	3.51586848485612 98
	3.55437609525768 98
	3.59288370565925 98.5
	3.63139131606082 98.5
	3.66989892646238 99.5
	3.70840653686395 99.5
	3.74691414726552 99.5
	3.78542175766708 99.5
	3.82392936806865 99.5
	3.86243697847021 100
	5 100
};
\end{groupplot}

\end{tikzpicture}

==> sections/asr_system.tex <==
%% Tex magic
% !TeX spellcheck = en_US
% !TeX encoding = utf-8
% !TeX root = interspeech_22.tex
% !TeX program = pdflatex
% !BIB program = bibtex

==> sections/deperecated_asr_experiments.tex <==
%% Tex magic
% !TeX spellcheck = en_US
% !TeX encoding = utf-8
% !TeX root = interspeech_22.tex
% !TeX program = pdflatex
% !BIB program = bibtex

% This part was transfered to secctions/experiments.tex

% \subsection{Source Separation}
% (Nur eine erste grobe Beschreibung damit ihr eine Idee habt, was ich mache)
% Source separation:

% Take the source activity information from the earlier systems and calculate an initialization for the posterior of the mixture model for a complete recording, i.e. the speech presence probability for each time frequency point.
% The number of classes is the given by the number of found speakers plus one. The additional class is introduced to model the noise. The noise is assumed to be always active.
% The initial value for the posterior is than simply the activity devided by the numer of active classes for each frame (i.e. broadcasted across the frequency).

% Mixture model: cACGMM with a time variant prior (normally frequency variant) for each frequency. The prior is shared between all frequencies. (Inline permutation solver is used, but most likely not nesseary).
% 20 iterations are done.

% The MM yield two information that are used in the followup processing: The a priori and a posterior probability. The a priori probability is used to identify the noise class: The most active class is rejected. (Probably unnecessary, because a class swap is unlikely).
% Further, the a priori probability is used to find segments of a single active speaker. The prior is smoothed with a max kernel that takes 79 values as input and a threshold of $0.5$.

% Extraction: Beamforming: Convolutional Beamformer (WPE+wMPDR).
% In each estimated segment, the posterior of the estimated speaker is used as mask to optain a speach PSD and the remaining masks, except the noise are used to calculate the distortion mask (At the moment: one minus speech, maybe no effct).


% \begin{table}[tbh]
%     % CB experiment root: /scratch/hpc-prf-nt1/cbj/deploy/cbj/egs/mmmeting/ref/mmmeting/<ID>
% 	\centering
% 	\caption{} 
% 	\begin{tabular}{ c c S[round-precision=2,round-mode=places, table-format = 2.2] }
% 		\toprule	
% 		\textbf{System} & \textbf{Signals}  &\textbf{WER / \%} \\
% 		\midrule
% 		- &Clean & \\
% 		- &Oracle Separation & \\
% 		\midrule
% 		Single-Ch. &Synchronous &\\
% 		\midrule
% 		\textcolor{gray}{Single-Array (Oracel Init.)} &Synchronous & 16.336184188403036 \\  % ID: 56
% 		Single-Array &Synchronous & 17.798975485635501 \\  % ID: 55
% 		\midrule
% 		\textcolor{gray}{Proposed (Oracel Init.)} &Synchronous & 13.916133298958672 \\  % ID: 60
% 		\textcolor{gray}{Proposed (Oracel Init.)} & Coarse Synchronized & 19.63390985618688 \\  % ID 61
% 		\textcolor{gray}{Proposed (Oracel Init.)} &Synchronized & 13.98675080985955 \\  % ID: 59
% 		Proposed &Synchronous & 14.065214710860524 \\  % ID: 58
% 		Proposed &Synchronized & 14.127985831661305 \\  % ID: 57
% 		\bottomrule
% 	\end{tabular}
% \end{table}

==> sections/intro.tex <==
%% Tex magic
% !TeX spellcheck = en_US
% !TeX encoding = utf-8
% !TeX root = interspeech_22.tex
% !TeX program = pdflatex
% !BIB program = bibtex

\section{Introduction}
\label{sec:intro}

\input{sections/sota_meeting_transcription}

==> sections/intro2.tex <==
%% Tex magic
% !TeX spellcheck = en_US
% !TeX encoding = utf-8
% !TeX root = interspeech_22.tex
% !TeX program = pdflatex
% !BIB program = bibtex

\section{Introduction}
\label{sec:intro}

This contribution is concerned with the transcription of meetings.
The meeting scenario considered here is characterized by long conversations among a small, however unknown, number of participants at fixed positions. Of those, none, one or even two speakers may be active at a time. 

Unlike most studies on meeting diarization~\cite{diary} and recognition~\cite{recognition}, we here consider an ad-hoc \gls{WASN} setup, where multiple initially unsynchronized microphone arrays at unknown positions are used for signal capture. We wish to take advantage of those multiple recording devices for improved diarization and recognition. 
This calls for signal synchronization, which consists of the subtasks, \gls{SRO} estimation, \gls{STO} estimation, and actual synchronization, i.e., alignment of the signals. \fromtgb{Not necessarily. A coarse sync + SRO compensation could also be used (see Araki). I do not see a real advantage of our system compared the Araki system. Our system is even blown up compared to their system but we have not shown that there is a real advantage compared to their work. They also use a spatial MM but in a different way.}
%Note that \gls{STO} estimation needs special consideration in a meeting scenario, because the observed \gls{TDOA} between two microphone signals consists of two contributions, the \gls{STO} caused by the devices to start recording at different moments in time, and the time of flight between the position of the currently active speaker and the microphones. 
%To disentangle the two contributions to the \gls{STO}, the geometry of the setup, i.e., the positions and orientations of the microphone arrays as well as the positions of the speakers, is estimated here. 
Thereby, the task of \gls{STO} estimation corresponds to the separation of the overall time shift between the signals recorded by different microphone arrays into the time shift which results from different recording start times of the microphone arrays, i.e., the \gls{STO}, and the \glspl{TDOF} of a signal emitted by a speaker to the distributed microphones (see~\cite{Gburrek22}).
For example, a physically correct \gls{STO} compensation enables to obtain the speakers' positions from the \gls{TDOF} information~\cite{DiBiase01}. 

\fromtgb{This argumentation is not really convincing but I also have no better idea.}
In \cite{Araki18}, also meeting recognition with asynchronous microphones is considered. However they  do not consider a physically correct \gls{STO} and geometry estimation and thus do not obtain position information, which here comes as a side effect. \fromrh{hat jemand besseres Argument?}

Given the position of the speakers and the synchronized signals, separation of overlapping speech and diarization can be carried out. 
Those two tasks are closely related and can be performed in different orders: separation-first or diarization-first \cite{Raj2021}.
The separation-first pipeline is motivated by the fact that many  diarization systems cannot cope appropriately with overlapping speech.
Therefore, the meeting  is first separated into non-overlapping streams, which is also termed \gls{CSS} \cite{20_Chen_LibriCSS}.
Then, utterance-boundaries of these separated streams are detected and speaker identities are assigned to each utterance via a diarization system. 
Other diarization systems are able to cope with overlapped speech, such that the order of processing can be reversed and source separation can benefit from diarization information. They typically employ neural speaker embeddings, either obtained from initial single-speaker segments  \cite{20_chime6_tsvad} or computed alongside diarization \cite{Fujita19}.

%Very good results are possible with both approaches. In particular, in the last CHIME-challenge \cite{20_watanabe_chime6} it was shown that a good speaker diarization allows the usage of model-based separation algorithms that result in impressive reductions in terms of the word error rate \cite{20_chime6_tsvad}.

%Both approaches can achieve good results.
% We here opt to do diarization first because we can take advantage of the position and activity information obtained from the previous synchronization step. With \gls{SRPPhaT} \cite{DiBiase01} we then obtain multi-speaker tracking and diarization information. Note, though,  that  one has to assume that the meeting participants occupy fixed positions. At least for more formal meetings that may not be a large restriction.

We here opt to do diarization first based on a multi-speaker tracking which is enabled by the physically correct \gls{STO} compensation.
There

The diarization estimate is used to initialize a spatial mixture model, whose outcome in turn is used to compute beamformer coefficients for source separation and signal enhancement. The enhanced signals are eventually forwarded to the speech recognizer.


%However, many current approaches to separation and diarization build upon synchronized audio streams, which are not given in realistic Ad-Hoc \gls{ASN} scenarios, where devices interconnect via wireless networks and each device has an independent \gls{ADC} clock.
%In such a scenario a synchronization has to compensate for a \gls{SRO} and \gls{STO} as discussed in \cite{Gburrek22}. While it is possible to view the synchronization decoupled from any other processing steps, doing so may discard information that can be useful for downstream tasks, e.g., the diarization as we will show later on.


The proposed system can thus be divided into the following sub-systems: (1) synchronization of the signals captured by the independent microphone arrays; (2) geometry calibration; (3) diarization;  and (4) speech enhancement and automatic speech recognition. \fromrh{(sollte mit den Farben in Fig. 2 uebereinstimmen)}

The paper is structured as follows. In the next section we give the problem statement. \cref{sec:system}  gives an overview of the overall system and then describes the individual system components \gls{SRO} and \gls{STO} estimation, where the latter utilizes the result of a geometry estimation component. 
%\fromrh{Den Satz würde ich an den Beginn von Kapitel 3.2 setzen:They are mainly based on the approach proposed in \cite{Gburrek22}: \glspl{SRO} are estimated by \gls{DWACD}, a method investigating the temporal change of the coherence between audio streams. \Gls{STO} estimation relies on the geometry estimation from \cite{GeoJournal}.} 
The geometry estimation system also provides  information about speaker activities, that, extended by the \gls{SRPPhaT} method, enables multi-speaker tracking and diarization on the synchronized audio streams, as described in \cref{subsec:srp}. The section concludes with a brief description of the source separation system. \Cref{sec:exp} presents the experimental evaluation.  To this end, we specifically simulate meeting scenarios where all participants occupy a fixed position around a conference table. Three compact microphone arrays are placed on the table and record the speakers' conversations independently, with the generated asynchronous audio streams containing realistic \gls{SRO} and \gls{STO} effects. 
The results obtained clearly demonstrate the benefits of using multiple arrays for both diarization and recognition. The paper is wrapped up with some conclusions drawn in \cref{sec:conclusions}.



==> sections/single_channel_diarization_baseline.tex <==
%% Tex magic
% !TeX spellcheck = en_US
% !TeX encoding = utf-8
% !TeX root = interspeech_22.tex
% !TeX program = pdflatex
% !BIB program = bibtex

==> sections/single_channel_separation_baseline.tex <==
%% Tex magic
% !TeX spellcheck = en_US
% !TeX encoding = utf-8
% !TeX root = interspeech_22.tex
% !TeX program = pdflatex
% !BIB program = bibtex

==> sections/sota_meeting_transcription.tex <==
%% Tex magic
% !TeX spellcheck = en_US
% !TeX encoding = utf-8
% !TeX root = interspeech_22.tex
% !TeX program = pdflatex
% !BIB program = bibtex

This contribution is concerned with the transcription of meetings. The meeting scenario considered is characterized by long conversations among a small, however unknown, number of participants. Of those, none, one or even two speakers may speak at a time. 
%Typically, such situations result in varying regions in the recording that contain either no speech, speech of a single speaker, or overlapping speech.
Unlike most studies on meeting diarization [] and recognition [], we here consider an ad-hoc setup, where multiple  initially unsynchronized microphone arrays at unknown positions are used for signal capture. We wish to take advantage of those for improved diarization and recognition.

Synchronization consists of the subtasks, \gls{SRO} estimation, \gls{STO} estimation, and resampling, i.e., alignment, of the signals. Note that \gls{STO} estimation needs special consideration in a meeting scenario, because the observed time difference of arrival between two microphone signals is not only caused by the \gls{STO} but also by the time of flight between the currently active speaker and the microphone.

In such a situation, meeting transcription can be divided the following sub-tasks:
(1) synchronization of the signals captured by the independent microphone arrays; (2) speaker activity estimation (diarization?); (3) speech separation and enhancement; and (4) automatic speech recognition.

The diarization and separation sub-tasks are closely related and can be performed in different orders: separation-first or diarization-first.
The separation-first pipeline is motivated by the fact that many state-of-the-art diarization and speech recognition systems are not build to handle overlapping speech, so that speech separation is required as a preprocessing step.
Therefore the meeting recording is first separated into non-overlapping streams, which is also termed \gls{CSS} \cite{20_Chen_LibriCSS}.
Then, utterance-boundaries of these separated streams are detected and speaker identities are assigned to each utterance via a diarization system. 
The diarization-first pipeline, on the other hand, first annotates which speaker is active when, and then uses this information for consecutive speech separation.

Very good results are possible with both approaches. In particular, in the last CHIME-challenge \cite{20_watanabe_chime6} it was shown that a good speaker diarization allows the usage of model-based separation algorithms that result in impressive reductions in terms of the word error rate \cite{20_chime6_tsvad}.
However, many current approaches to separation and diarization build upon synchronized audio streams, which are not given in realistic Ad-Hoc \gls{ASN} scenarios, where devices interconnect via wireless networks and each device has an independent \gls{ADC} clock.
In such a scenario a synchronization has to compensate for a \gls{SRO} and \gls{STO} as discussed in \cite{Gburrek22}. While it is possible to view the synchronization decoupled from any other processing steps, doing so may discard information that can be useful for downstream tasks, e.g., the diarization as we will show later on.

In this contribution, we specifically simulate meeting scenarios where all participants occupy a fixed position around a conference table. Three compact microphone arrays are placed on the table and record the speakers' conversations independently, with the generated non-synchronous audio streams containing realistic \gls{SRO} and \gls{STO} effects. We propose a meeting transcription system that extends the diarization-first pipeline to perform all steps from synchronisation, diarization, and separation to finally transcription. So instead of using a dedicated diarization module, we propose a system for joint stream synchronization and diarization.
Estimating \glspl{SRO} and \glspl{STO} from audio streams is mainly based on the approach proposed in \cite{Gburrek22}: \glspl{SRO} are estimated by \gls{DWACD}, a method investigating the temporal change of the coherence between audio streams. \gls{STO} estimation requires the knowledge about the geometry of the setup, i.e., the positions and orientations of the microphone arrays as well as the positions of the speakers. 
We show geometry estimation from non-synchronous audio streams, even in presence of speaker changes and overlapping speech utterances from different speaker positions. 
Thereby, the geometry estimation system not only enables solving the \gls{STO} task, but it also provides a precise information about speaker activities, which extended by a SRP-PHAT method enable multi-speaker tracking and diarization on the synchronized audio streams.
Afterwards, the diarization estimate is used to initialize a spatial mixture model that separates each meeting into a single output per speaker. The aim of this paper is to show that the distributed nature of the \gls{WASN} can lead to an improved source separation, diarization and meeting transcription compared to a single microphone or a single compact microphone array.

This paper is structured as follows: \fromtcl{TODO: Mit RH klären, ob es gestrichen werden kann}
%TS-VAD + GSS
%        Intro Meeting-scenario (ad-hoc / multiple devices)
%        Processing Pipeline (CSS + Dia-First)
%        TS-VAD + GSS
%        Notwendigkeit der Synchronisaion
%        Motivation: Verwendung von SRO-STO Infos zur räumlichen Diarization
%       Ansatz beschreiben
%       Struktur des Papers
